Multi-VQG: Generating Engaging Questions for Multiple Images

Generating engaging content has drawn much recent attention in the NLP community. Asking questions is a natural way to respond to photos and promote awareness. However, most answers to questions in traditional question-answering (QA) datasets are factoids, which reduce individuals' willingness to answer. Furthermore, traditional visual question generation (VQG) confines the source data for question generation to single images, resulting in a limited ability to comprehend time-series information of the underlying event. In this paper, we propose generating engaging questions from multiple images. We present MVQG, a new dataset, and establish a series of baselines, including both end-to-end and dual-stage architectures. Results show that building stories behind the image sequence enables models to generate engaging questions, which confirms our assumption that people typically construct a picture of the event in their minds before asking questions. These results open up an exciting challenge for visual-and-language models to implicitly construct a story behind a series of photos to allow for creativity and experience sharing and hence draw attention to downstream applications.

==> figures/answer_compare.tex <==
\begin{figure}[t!]
    \centering
    
    \hfill
    \begin{subfigure}{0.19\textwidth}
    \includegraphics[width=\textwidth]{answer_length.pdf}
    % \vspace{-1.5pc}
    \caption{}
    \label{fig:ans_len}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.19\textwidth}
    \includegraphics[width=\textwidth]{answer_similarity.pdf}
    % \vspace{-1.7pc}
    \caption{}
    \label{fig:ans_sim}
    \end{subfigure}
    \hfill
    % \vspace{-0.8pc}
	\caption{Comparison of answer quality among different setups. (a) Average sentence length (b) Average cosine similarity among five answers.}
    % \vspace{-1.2pc}
    \label{fig:compare_a}
\end{figure}

==> figures/answer_wordcloud.tex <==
\begin{figure}[t!]
    \centering
    
    % \includegraphics[width=0.48\textwidth]{answer_wordcloud.pdf}
    \hfill
    \begin{subfigure}{0.20\textwidth}
    \includegraphics[width=\textwidth]{answer_wordcloud_VIST_1_answer.pdf}
    % \vspace{-1.5pc}
    \caption{$VIST_1$}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.20\textwidth}
    \includegraphics[width=\textwidth]{answer_wordcloud_VIST_5_answer.pdf}
    % \vspace{-1.5pc}
    \caption{$VIST_5$}
    \end{subfigure}
    \hfill
    
    \hfill
    \begin{subfigure}{0.20\textwidth}
    \includegraphics[width=\textwidth]{answer_wordcloud_VQG_orig_answer.pdf}
    % \vspace{-1.5pc}
    \caption{$VQG_{orig}$}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.20\textwidth}
    \includegraphics[width=\textwidth]{answer_wordcloud_VQG_our_answer.pdf}
    % \vspace{-1.5pc}
    \caption{$VQG_{ours}$}
    \end{subfigure}
    \hfill
    
	\caption{The wordcloud of answers corresponding to different questions settings. The top 100 frequent words in answers are shown in each wordcloud.}
% 	\vspace{-1.2pc}
    \label{fig:ans_wordcloud}
\end{figure}

==> figures/question_compare.tex <==
\begin{figure*}[t!]
    \centering
    \hfill
    \begin{subfigure}{0.15\textwidth}
    \includegraphics[width=\textwidth]{vocab_size.pdf}
    % \vspace{-1.5pc}
    \caption{}
    \label{fig:vocab_size}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.15\textwidth}
    \includegraphics[width=\textwidth]{question_length.pdf}
    % \vspace{-1.5pc}
    \caption{}
    \label{fig:q_len}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.15\textwidth}
    \includegraphics[width=\textwidth]{syntactic_complexity.pdf}
    % \vspace{-1.5pc}
    \caption{}
    \label{fig:syntactic_complexity}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.15\textwidth}
    \includegraphics[width=\textwidth]{percentage_of_abstract_term.pdf}
    % \vspace{-1.5pc}
    \caption{}
    \label{fig:abs_term}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.15\textwidth}
    \includegraphics[width=\textwidth]{average_term_depth.pdf}
    % \vspace{-1.5pc}
    \caption{}
    \label{fig:term_depth}
    \end{subfigure}
    \hfill
    % \vspace{-0.5pc}
	\caption{Comparison of question quality among different setups. (a) Vocabulary size. (b) Average sentence length. (c)
Syntactic Complexity. (d) Percentage of abstract terms. (e) Average term depth.}
    % \vspace{-.5pc}
    \label{fig:compare_q}
\end{figure*}

==> tables/human_ranking.tex <==
\begin{table*}[t]
    \centering
    \small
    \begin{tabular}{clccccc}
        \toprule
        Group & Baseline & Benchmark~1 & Benchmark~2 & Benchmark~3 & Benchmark~4 & Benchmark~5 \\
        \midrule
        \midrule
        
        \multirow{3}{*}{1} & $\text{VL-T5}_\text{F\_VIST}$ & \textbf{35.08} (\textbf{1.981}) & \textbf{34.80} (\textbf{1.985}) & 34.60 (1.983) & \textbf{35.04} (\textbf{1.971}) & \textbf{35.80} (\textbf{1.963}) \\
        & $\text{VL-T5}_\text{F\_VCR}$ & 31.84 (2.038) & 32.64 (2.018) & 30.64 (2.050) & 32.60 (2.026) & 30.12 (2.058) \\
        & $\text{VL-T5}_\text{F\_VQG}$ & 33.08 (1.981) & 32.56 (1.995) & \textbf{34.76} (\textbf{1.966}) & 32.36 (2.001) & 34.08 (1.978) \\
        \midrule
        
        \multirow{3}{*}{2} & $\text{CAP2Q}_\text{CLIP}$ & 33.44 (2.016) & \textbf{33.96} (2.019) & 32.88 (2.020) & \textbf{34.24} (\textbf{1.986}) & 33.20 (2.001) \\
        & $\text{STY2Q}_\text{CLIP}$ & \textbf{33.44} (2.006) & 32.80 (1.995) & 33.36 (2.001) & 31.64 (2.025) & 33.32 (2.002) \\
        & $\text{SUM2Q}_\text{CLIP}$ & 33.12 (\textbf{1.977}) & 33.24 (\textbf{1.985}) & \textbf{33.76} (\textbf{1.979}) & 34.12 (1.988) & \textbf{33.48} (\textbf{1.996}) \\
        \midrule
        
        \multirow{3}{*}{3} & $\text{STY2Q}_\text{CLIP}$ & 34.09 (1.988) & \textbf{34.81} (\textbf{1.974}) & \textbf{34.13} (\textbf{1.984}) & 32.01 (2.022) & \textbf{33.97} (\textbf{1.993}) \\
        & $\text{VL-T5}_\text{F\_VIST}$ & \textbf{34.25} (\textbf{1.976}) & 32.97 (2.012) & 32.97 (2.008) & 33.89 (\textbf{1.980}) & 32.13 (2.008) \\
        & $\text{VL-T5}_\text{C}$ & 31.65 (2.036) & 32.21 (2.012) & 32.89 (2.008) & \textbf{34.09} (1.998) & 33.89 (1.999) \\
        \midrule
        
        \multirow{2}{*}{4} & $\text{VL-T5}_\text{F\_VIST}$ & \textbf{50.68} (\textbf{1.493}) & \textbf{51.24} (\textbf{1.488}) & \textbf{50.48} (\textbf{1.495}) & \textbf{50.48} (\textbf{1.495}) & 49.28 (1.507) \\
        & $\text{VL-T5}_\text{A\_VIST}$ & 49.32 (1.507) & 48.76 (1.512) & 49.52 (1.505) & 49.52 (1.505) & \textbf{50.72} (\textbf{1.493}) \\
        \bottomrule
    \end{tabular}
    % \vspace{-.5pc}
    \caption{Human evaluation of different groups for five benchmarks. 
    Group~1: end-to-end baselines pretrained on different datasets. 
    Group~2: dual-stage baselines with different types of text as input. 
    Group~3: baselines with or without story information.
    Group~4: end-to-end baselines with fine-tuning or adapt-tuning. 
    Given methods and benchmarks by row and column, the percentage indicates the ratio of rank-1 questions among all questions (higher is better). The number in brackets is the average ranking among all questions (lower is better).}
    % \vspace{-.5pc}
    \label{tb:human_eval}
\end{table*}
